High-Energy Cosmic-Ray Propagation in the Milky Way and the Associated Diffuse Gamma-Ray Emission

Simulations of Galactic CR transport were performed with the software GALPROP, with the resulting gamma-ray flux calculated up to the PeV regime. The impact of altering parameters such as the number and distribution of CR sources, the distribution of infrared radiation between stars, and the distribution and strength of the Galactic magnetic field (GMF), were investigated. For the first time the modelling variation in the TeV predictions due to uncertainties in the Galactic distributions was quantified. Additionally, the modelling variation from considering a stochastic placement of the CR sources was quantified up to 1 PeV. The simulation results were compared to the most detailed Galactic TeV gamma-ray survey: the H.E.S.S. Galactic plane survey (HGPS). The GALPROP predictions were broadly compatible with the large-scale emission from the HGPS after accounting for both the catalogued sources and estimates of the unresolved source fraction. At 1 TeV the gamma-ray emission from CR electrons was found to contribute $\sim$50\% to the large-scale emission. The GMF was found to be an important modelling consideration above 1 TeV as it impacted the large-scale emission by approximately a factor of two. Additionally, the CR electron flux at Earth above 1 TeV was found to vary by over a factor of ten over a period of a few million years due. The GALPROP models were found to agree with observations of the diffuse gamma rays in the TeV regime by H.E.S.S., and the PeV regime by LHAASO, extending the demonstrated accuracy of GALPROP into the TeV--PeV regime. The results will also inform the next generation of experiments, such as the Cherenkov telescope array (CTA), on possible observation strategies and background considerations. It was also found that the proposed CTA Galactic plane survey will be sensitive enough to observe the large-scale diffuse gamma-ray emission in the TeV regime.

==> mainmatter/chapter_4/4_figures/_rounded_square_diagram.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        
        % Draw a large square
        \draw[thick] (0,0) -- (0,7) -- (7,7) -- (7,0) -- (0, 0);
        % Fill the square with grey to create a shaded region
        \fill[black!10!white] (0,0) -- (0,7) -- (7,7) -- (7,0) -- (0, 0);
        
        % Draw a quarter-circle for each corner and then fill it
        % (x,y) is the point where the arc begins
        % (t1,t2,r) is the start angle, end angle, and radius
        \draw[thick] (0,2) arc (180:270:2);
        \fill[white] (0,2) arc (180:270:2);
        \draw[thick] (2,7) arc (90:180:2);
        \fill[white] (2,7) arc (90:180:2);
        \draw[thick] (7,5) arc (0:90:2);
        \fill[white] (7,5) arc (0:90:2);
        \draw[thick] (5,0) arc (270:360:2);
        \fill[white] (5,0) arc (270:360:2);
        
        % Fill the remaining shape
        \fill[white] (0,2) -- (0,5) -- (2,7) -- (5,7) -- (7,5) -- (7,2) -- (5,0) -- (2,0) -- (0,2);
        
        % Draw a small square in the centre
        \draw[thick] (2,2) -- (2,5) -- (5,5) -- (5,2) -- (2, 2);

        % Dashed line from small square to large square
        \draw[thick, dashed] (5,5) -- (7,5);
        
        % Add text
        \node at (3.5,2.3) {$l=0.1145^{\circ}$};
        \node at (3.5,0.3) {$l+2R_{c}$};
        \node at (6,5.3) {$R_{c}$};
        
    \end{tikzpicture}
    \hfil
    \begin{tikzpicture}
        
        % Draw a large square
        \draw[thick] (0,0) -- (0,7) -- (7,7) -- (7,0) -- (0, 0);
        % Fill the square with grey to create a shaded region
        \fill[black!10!white] (0,0) -- (0,7) -- (7,7) -- (7,0) -- (0, 0);
        
        % Draw a quarter-circle
        \draw[thick] (7,0) arc (0:90:7);
        % Fill the arc with white, which will be placed on top of the grey square
        \fill[white] (7,0) arc (0:90:7);
        
        % Filling the arc leaves a triangle of grey behind. Fill that area with white
        \fill[white] (0,0) -- (0,7) -- (7,0) -- (0, 0);
        
        % Add labels
        \node at (3.5,0.3) {Radius, $R_{c}$};
        % Add labels
        \node at (6,6.5) {$A_{\text{shaded}}$};
        
    \end{tikzpicture}
    
    \caption{Diagram of a rounded square, where $l$ is the side length of the \hpx{} pixel and $R_{c}$ is the telescope beam radius. The outer square has side lengths $l+2R_{c}$. The area of the full averaging region can be found by subtracting the area of the shaded regions from the outer square, and the area of the shaded regions can be found by subtracting a quarter of the beam area from the square with side lengths $R_{c}$.}
    \label{fig:rounded_square}
    
\end{figure}
